Integrating Usage Control into Distributed Ledger Technology for Internet of Things Privacy

The Internet of Things brings new ways to collect privacy-sensitive data from billions of devices. Well-tailored distributed ledger technologies (DLTs) can provide high transaction processing capacities to IoT devices in a decentralized fashion. However, privacy aspects are often neglected or unsatisfying, with a focus mainly on performance and security. In this paper, we introduce decentralized usage control mechanisms to empower IoT devices to control the data they generate. Usage control defines obligations, i.e., actions to be fulfilled to be granted access, and conditions on the system in addition to data dissemination control. The originality of this paper is to consider the usage control system as a component of distributed ledger networks, instead of an external tool. With this integration, both technologies work in synergy, benefiting their privacy, security and performance. We evaluated the performance improvements of integration using the IOTA technology, particularly suitable due to the participation of small devices in the consensus. The results of the tests on a private network show an approximate 90% decrease of the time needed for the UCS to push a transaction and make its access decision in the integrated setting, regardless of the number of nodes in the network.

==> Images/cover_letter_reviewer.tex <==
DATE,

Dear Dr. Xu Yuan, Prof. Honggang Wang, dear reviewers,

We are writing to submit our revised manuscript entitled \emph{Integrating Usage Control into Distributed Ledger
Technology for Internet of Things Privacy}. We thank the reviewers and editors for their valuable feedback and constructive comments on our original submission.

In response to the reviewers' comments, we have made substantial revisions to the manuscript, specifically addressing the flaws that were identified in the original article. We have carefully analyzed the issues raised by the reviewers and have provided the following answers to the requests, underlined in the document:

\textbf{Reviewer 1}:
\begin{enumerate}
   \item \emph{You should provide more discussions about your contributions in the Introduction}.
    \item[R1] $\to$ we added a discussion about the contributions of the article at the end of the introduction, before the outline of the document;
   \item \emph{It will be better if you present Fig. 1 with more descriptions
of its workflow};
   \item[R2] $\to$ we added the workflow between the different components of the usage control system, with the associated messages;
   \item \emph{I think the Background is a little bit redundant. You can present it with less space};
   \item[R3] $\to$ 1) We removed the discussion about consortium blockchains, not mentioned again in the article (II.B). 2) We also removed a paragraph about the UCS distribution, which is never used in the article and could be considered related work. (II.A) 3) We removed the paragraph about why usage control is a PET (II.A). This paragraph is obsolete with the more accurate privacy evaluation (VII) and redundant as it repeats the beginning of section II.A ;
   \item \emph{Could you please evaluate the main selling point of this work,
i.e., privacy protection, with some experiments? The presented
results cannot convince me that your claimed contributions are
solid};
\item[R4] $\to$ Usage control being a privacy-enhancing technology, a privacy assessment is indeed expected. While the review explicitly asks for experiments, it is hard to implement relevant, non-trivial tests. Most of the experiments would actually measure the performance of the usage control system, e.g., are the policies properly enforced by the usage control system, even under high load? Rather than experiments, we believe the comment (the need to evaluate privacy protection) is better addressed by providing a thorough privacy risk assessment. We provide such analysis in the new section VII, using the LINDDUN framework;
\end{enumerate}


\textbf{Reviewer 2}:
\begin{enumerate}
\item \emph{In section 2.A the definition of “conditions” is not
straightforward};
\item[R1] $\to$ The definition of condition has been extended, and examples of both obligations and conditions have been provided for clarity in 2.A;
\item \emph{In section 2.B, IOTA 2.0 is mentioned, but it is not clear why
the PoW is not necessary since its role is to prevent spam};
\item[R2] $\to$ The rate control mechanism, replacing the proof of work, is now introduced in II.C as well as its main purpose: managing overload;
\item \emph{In section 2.B, the sentence “Besides, some cryptocurrencies do
not build their transaction graphs as a chain but using different
graphs” is not very clear. In the literature, transaction graphs
are often referred to as graphs where nodes are DLT accounts,
while edges are transactions from a node toward another node.}
\item[R3] $\to$ The term "transaction graph" is definitely equivocal in the article. Transaction graph usually refers in the literature to the representation of transactions (edges) between addresses (sets). The transaction graphs in this article were actually transactions (sets) referring to other transactions using edges. For disambiguation purposes, "transaction graph" is replaced by the correct term "transaction ledger" or "ledger type" (II.A, IV.A);
\item \emph{In section 3.A, the sentence “The main reason stated by the
authors is the continuous monitoring of the data access, thanks to
attribute mutability” is not clear};
\item[R4] $\to$ The sentence is detailed (III.A) and now also explains not only the purpose of usage control, but why a private blockchain is used;
\item \emph{In section 3.A, the sentence “Ethereum is not an IoT-friendly
blockchain when the number of transactions is high, as it uses the
proof of work, or the proof of stake in its upcoming version 2.0”
is not entirely true, as currently PoW version of Ethereum is
deprecated;}
\item[R5] $\to$ The switch to proof of stake is indeed completed since September 15, 2022, and proof of work is deprecated. The sentence was removed;
\item \emph{In section 4.A, the impact of transaction graphs on equitability
and decentralization is not clear. Again, I think there is just a
misuse of the term “transaction graph”}.
\item[R6] $\to$ Same as R3, transaction graph is indeed misused, replaced by transaction ledger in IV.A;
\item \emph{In section 4.B, the sentence “a higher number of nodes makes
some attacks harder, such as the 51\% attack” is not valid for
DAGs, as far as I know. In fact, the 51\% is linked to the
willingness of the attackers to gain the reward for validating a
block and to control the flow of transactions in the DLT. However,
some of these dynamics cannot occur in a DAG-based DLT.};
\item[R7] $\to$ The mention of the 51\% attack is not accurate enough because the tolerance in DAG-based networks is lower (33\%). However, while mining does not exist as such, having 33\% of the network computing power still enables it to carry out attacks, notably double spending. The name of the attack is corrected in IV.B, and citation is provided specifically for the DAG;
\item \emph{In section 4.B, it is not very clear what for auditability is meant;}
\item[R8] $\to$ The purpose of auditability has been split into the benefit for data owners and for data readers (IV.B), which should highlight be clearer;
\item \emph{In section 4.C, the management of data encryption is not very clear. A database management system is mentioned, but its role is
not explained;}
\item[R9] $\to$ The term "distributed management system" and the reference to encryption may be confusing. We emphasized the fact that encryption is not used in our solution, and that the purpose of the database is to store the data that must not be publicly available (section IV.C);
\item \emph{In section 5.B, it is more correct to say “company that wants”
instead of “company who wants”};
\item[R10] $\to$ The sentence was corrected;
\item \emph{In section 6.A, it is said that devnet is used for testing but
also that “it does not allow to reproduce the tests as the
network is modified with updates”. This concept is not clear};
\item[R11] $\to$ We added details about why the tests can not be reproduced on the public development network of IOTA, notably because the topology can not be controlled, and the network can completely change with updates (section VI.A);



\end{enumerate}

Thank you for your consideration.

Sincerely,
Nathanaël Denis,
\emph{nathanael.denis@telecom-sudparis.eu}.
PhD student at Télécom SudParis, Institut Polytechnique de Paris, member of the chair Values and Policies of Personal Information
On behalf of the coauthors.

